A smart electric bike for smart cities

This is a Masters Thesis completed at University College Dublin, Ireland in 2017 which involved augmenting an off-the-shelf electric bike with sensors to enable new services to be delivered to cyclists in cities. The application of primary interest was to control the cyclist's ventilation rate based on the concentration of local air pollutants. Detailed modelling and system design is presented for our Cyberphysical system which consisted of a modified BTwin e-bike, Cycle Analyst sensors, the cyclist themselves, a Bluetooth connected smartphone and our algorithms. Control algorithms to regulate the proportion of power the cyclist provided as a proxy for their ventilation rate were proposed and validated in a basic way, which were later proven significantly further in Further Work (see IEEE Transactions on Intelligent Transportation Systems paper: https://ieeexplore.ieee.org/abstract/document/8357977). The basic idea was to provide more electrical assistance to cyclists in areas of high air pollution to reduce the cyclist ventilation rate and thereby the amount of air pollutants inhaled. This presents an interesting control challenge due to the human-in-the-loop characteristics and the potential for impactful real life applications. A background literature review is provided on energy as it relates to cycling and some other applications are also discussed. A link to a video which demonstrates the system is provided, and also to a blog published by IBM Research about the system.

==> back-matter/vita.tex <==
\chapter*{Vita} \label{ch:vita}
Vita goes here...

	Contact details for author

 Its purpose is to give a bit of background about the author.
 A vita is the equivalent of a resume, and is used to list your educational and professional qualifications. 
 Your vita may follow one of two formats:
 
 Narrative
 Traditional CV (resume) style
 The narrative contains personal, academic, and professional information about the author written in biographical form.  It is similar to the biographical narratives found in books by your favourite authors. 
 
 The traditional CV (resume) style is the most common format used.  It is a methodical listing of your professional and educational experiences, including any research projects and publications you've contributed to.  There is no required format for this style.  Instead, you may arrange the contents in the manner that best suits your academic field as long as the general format for theses and dissertations is followed.

==> front-matter/nomenclature.tex <==
% enter the list of nomenclature here
%\nomenclature{$r$}{Radial coordinate}
%\nomenclature{$\theta$}{Tangential coordinate}
%\nomenclature{$z$}{Axial coordinate}
%\nomenclature{$\bar{}$}{Denotes a dimensional variable}
%\nomenclature{$\psi$}{Streamfunction}
%\nomenclature{$u_r$}{Radial velocity}%
%\nomenclature{$u_{\theta}$}{Tangential velocity}%
%\nomenclature{$u_z$}{Axial velocity}%
%\nomenclature{$p$}{Pressure} 


==> front-matter/nomenclature2.tex <==
\chapter*{Nomenclature}

\begin{centering}

%\begin{tabular}{ll}
%\textbf{ACR} & \textbf{A}ir \textbf{C}hange \textbf{R}ate\\
%\textbf{BEM} & \textbf{B}uilding \textbf{E}nergy\textbf{M}odel\\
%\textbf{BEPS} & \textbf{B}uilding \textbf{E}nergy \textbf{P}erformance \textbf{S}imulation\\
%\textbf{CC} & \textbf{C}ontinuous \textbf{C}ommissioning\\
%\textbf{COP} & \textbf{C}oefficient \textbf{O}f \textbf{P}erformance\\
%\textbf{DEAP} & \textbf{D}welling \textbf{E}nergy \textbf{A}ssessment \textbf{P}rocedure\\
%\textbf{DEC} & \textbf{D}isplay \textbf{E}nergy \textbf{C}ertificate\\
%\textbf{DHW} & \textbf{D}omestic \textbf{H}ot \textbf{W}ater\\
%\textbf{DSA} & \textbf{D}ifferential \textbf{S}ensitivity \textbf{A}nalysis\\
%\textbf{GSA} & \textbf{G}lobal \textbf{S}ensitivity \textbf{A}nalysis\\
%\textbf{GSHP} & \textbf{G}round \textbf{S}ource \textbf{H}eat \textbf{P}ump\\
%\textbf{HHV} & \textbf{H}igher \textbf{H}eating \textbf{V}alue\\
%\textbf{IC} & \textbf{I}nfluence \textbf{C}oefficient\\
%\textbf{IR} & \textbf{I}nfiltration \textbf{R}ate\\
%\textbf{LHV} & \textbf{L}ower \textbf{H}eating \textbf{V}alue\\
%\textbf{MCA} & \textbf{M}onte \textbf{C}arlo \textbf{A}nalysis\\
%\textbf{PCM} & \textbf{P}hase \textbf{C}hange \textbf{M}aterials\\
%\textbf{ROM} & \textbf{R}educed \textbf{O}rder \textbf{M}odel\\
%\textbf{HHV} & \textbf{H}igher \textbf{H}eating \textbf{V}alue\\
%\textbf{SA} & \textbf{S}ensitivity \textbf{A}nalysis\\
%\textbf{WWR} & \textbf{W}indow to \textbf{W}all \textbf{R}atio\\
%\end{tabular}

\end{centering}

==> front-matter/quote.tex <==
\chapter*{}
{\it Some quotation...}
